The Luminosity Dependence of the Galaxy Merger Rate

We measure the number of companions per galaxy (Nc) as a function of r-band absolute magnitude for both the Sloan Digital Sky Survey and the Croton et al. (2006) semi-analytic catalog applied to the Millennium Run simulation. For close pairs with projected separations of 5-20 h^{-1} kpc, velocity differences less than 500 km/s, and luminosity ratios between 1:2 and 2:1, we find good agreement between the observations and simulations, with Nc consistently close to 0.02 over the range -22 < M_r < -18. For larger pair separations, Nc(M_r) instead becomes increasingly steep towards the faint end, implying that luminosity-dependent clustering plays an important role on small scales. Using the simulations to assess and correct for projection effects, we infer that the real-space Nc(M_r) for close pairs peaks at about M*, and declines by at least a factor of two as M_r becomes fainter. Conversely, by measuring the number density of close companions, we estimate that at least 90% of all major mergers occur between galaxies which are fainter than L*. Finally, measurements of the luminosity density of close companions indicate that L* galaxies likely dominate in terms of the overall importance of major mergers in the evolution of galaxy populations at low redshift.

==> tab1.tex <==
\begin{table}
\begin{center}
\caption{SDSS Host Galaxies
\label{tabhost}}
\begin{tabular}{cccccc}
\tableline\tableline
Host ObjID
%%\footnote{Print version contains only the top five entries.  
%%Electronic edition to contain complete list of SDSS Host Galaxies.}
&RA&Dec&$z$&$M_r$&Companion ObjID\\
\tableline
%\input{hosts-mini}
587724198275842071&10.610426&14.70509&0.05539&$-19.72$&587724198275842073\\
587724197207670886&23.645067&13.18706&0.06304&$-20.17$&587724197207670885\\
587724197207670885&23.646278&13.18500&0.06226&$-20.50$&587724197207670886\\
587731513153159200&42.731424&0.36690&0.04384&$-20.10$&587731513153159199\\
587731513153159199&42.739416&0.36940&0.04423&$-19.76$&587731513153159200\\
588015510362718334&44.756365&0.89605&0.13359&$-21.63$&588015510362718335\\
587731511544316024&46.847470&-1.01978&0.08385&$-20.65$&587731511544316025\\
587731512082104440&48.939335&-0.49559&0.08698&$-20.75$&587731512082104439\\
587731512082104439&48.940395&-0.49697&0.08703&$-21.50$&587731512082104440\\
587731512082890888&50.701675&-0.62018&0.03664&$-19.57$&587731512082890786\\
587731512082890786&50.707936&-0.61237&0.03534&$-19.44$&587731512082890888\\
587725470662001002&115.346035&37.55974&0.08488&$-20.56$&587725470662001003\\
587738947193340000&116.788372&17.20457&0.07514&$-20.21$&587738947193340002\\
588016878285292076&116.798143&18.06763&0.05029&$-19.22$&588016878285292061\\
587738371667788442&116.946409&17.06907&0.09940&$-20.77$&587738371667788441\\
587738371667788441&116.947992&17.07127&0.09993&$-21.39$&587738371667788442\\
588016878285816131&117.648011&18.82647&0.06866&$-20.04$&588016878285816132\\
587732156314484989&117.916895&24.07732&0.06147&$-20.37$&587732156314484990\\
587732156314484990&117.921072&24.08094&0.06092&$-20.16$&587732156314484989\\
587739377227399701&117.988736&15.64036&0.10286&$-20.89$&587739377227399700\\
587725551731146928&118.176110&43.74835&0.10508&$-20.94$&587725551731146927\\
587725551731146927&118.179010&43.74851&0.10479&$-21.45$&587725551731146928\\
587734840668782942&118.669669&23.05716&0.09240&$-20.76$&587734840668782941\\
587734840668782941&118.670754&23.05917&0.09080&$-20.57$&587734840668782942\\
587728668803793221&119.640629&37.78050&0.03862&$-18.91$&587728668803793217\\
587728668803793217&119.646067&37.77625&0.03954&$-18.77$&587728668803793215\\
587728668803793217&119.646067&37.77625&0.03954&$-18.77$&587728668803793221\\
587727865644777756&119.686944&37.36505&0.03973&$-18.83$&587727865644777755\\
587727865644974418&119.884562&37.88877&0.04053&$-19.09$&587727865644974417\\
587732053237039195&120.418737&28.61421&0.07848&$-20.68$&587732053237039194\\
587732053237039194&120.419150&28.61057&0.07914&$-20.67$&587732053237039195\\
588007005769957428&120.521020&44.00681&0.07517&$-20.85$&588007005769957426\\
587739115772510497&121.387114&19.33825&0.12439&$-21.31$&587739115772510496\\
587739115772510496&121.388895&19.33839&0.12399&$-21.54$&587739115772510497\\
588007004696281213&121.527910&43.66047&0.06336&$-20.17$&588007004696281210\\
588007004696281210&121.533480&43.65629&0.06360&$-20.66$&588007004696281213\\
587727865646088532&121.925355&39.81711&0.06838&$-20.80$&587727865646088533\\
587727865646088533&121.925944&39.81150&0.06862&$-20.24$&587727865646088532\\
587735235808788553&123.265390&24.55854&0.02078&$-18.22$&587735235808788552\\
587725552809279538&125.762891&52.39291&0.03400&$-18.44$&587725552809279539\\
587725552809279539&125.768339&52.39469&0.03382&$-19.08$&587725552809279538\\
587735344791683448&125.918537&7.15410&0.08143&$-20.39$&587735344791683447\\
587725979614773457&127.315605&50.75436&0.11726&$-21.69$&587725979614773458\\
587725979614773458&127.317243&50.75467&0.11828&$-21.36$&587725979614773457\\
588010137337069703&128.330953&47.84514&0.13346&$-21.96$&588010137337069704\\
588010137337069704&128.331789&47.84637&0.13332&$-21.45$&588010137337069703\\
587734621631086790&129.573312&30.91486&0.04765&$-20.34$&587734621631086789\\
587732469850767564&129.716462&33.20872&0.06964&$-20.56$&587732469850767563\\
587732469850767563&129.718149&33.20740&0.06973&$-21.16$&587732469850767564\\
587739115776835600&130.350941&24.49508&0.04299&$-19.21$&587739115776835601\\
588016878292500646&131.224965&27.71900&0.08543&$-21.24$&588016878292500647\\
588016878292500647&131.225904&27.72000&0.08378&$-21.23$&588016878292500646\\
587735043076391111&131.289744&30.18779&0.07794&$-20.79$&587735043076391112\\
587732052705476746&131.316508&36.51920&0.07634&$-20.29$&587732052705476745\\
587732052705476745&131.318730&36.51937&0.07628&$-20.49$&587732052705476746\\
587725471207260240&131.360504&53.15447&0.03057&$-18.15$&587725471207260238\\
588297863640842460&133.033976&33.14354&0.06649&$-20.10$&587734621632725182\\
588016841249390716&133.371282&30.27869&0.07137&$-20.37$&588016841249390715\\
587735240638791876&133.383723&31.62926&0.07197&$-20.33$&587735240638791875\\
587735240638791875&133.385870&31.62490&0.07301&$-20.99$&587735240638791876\\
587726032228253901&133.616406&1.19695&0.05841&$-20.04$&587726032228253899\\
587726032228253899&133.617490&1.20203&0.05853&$-20.40$&587726032228253901\\
587738946664530084&133.627940&26.97758&0.06054&$-19.82$&587738946664530083\\
587732482732523688&133.643775&35.88369&0.07789&$-20.55$&587732482732523689\\
587727942953402590&134.529973&1.10463&0.07253&$-20.22$&587727942953402591\\
588007005776183456&134.591601&54.96826&0.08915&$-20.56$&588007005776183457\\
588013382728221044&134.930187&39.42908&0.09537&$-21.08$&588013382728221046\\
588848900966777144&135.141101&0.76015&0.07063&$-20.83$&588848900966777145\\
588848900966777145&135.144529&0.75798&0.07083&$-20.39$&588848900966777144\\
587725979617919091&135.420727&56.10503&0.14105&$-21.87$&587725979617919092\\
587735240103100624&136.449920&32.78217&0.06356&$-19.85$&587735240103100625\\
588010136266277051&136.810200&52.06205&0.05952&$-19.84$&588010136266277052\\
588009365861630106&137.299717&50.92415&0.02933&$-18.91$&588009365861630126\\
588009365861630126&137.305129&50.93596&0.02901&$-18.80$&588009365861630106\\
588017977802096689&138.471458&29.07810&0.05342&$-20.21$&588017977802096690\\
588017977802096690&138.475813&29.08074&0.05360&$-19.78$&588017977802096689\\
587734621635149881&138.760417&36.08991&0.07104&$-20.21$&587734621635149882\\
588016890631946322&138.842018&31.35558&0.06336&$-20.75$&588016890631946323\\
588016890631946323&138.847035&31.35205&0.06353&$-20.31$&588016890631946322\\
587732578300723432&139.164913&5.42990&0.14348&$-21.73$&587732578300723431\\
587732483809280204&140.122478&40.44390&0.07367&$-20.17$&587732483809280205\\
587735661008781533&141.414356&32.80388&0.05218&$-19.60$&587735661008781534\\
587732152030527507&141.597377&39.92256&0.12136&$-21.29$&587732152030527508\\
588009366937272473&141.786954&54.37495&0.12688&$-21.33$&588009366937272472\\
587734949661769846&143.405698&9.85351&0.04992&$-19.89$&587734949661769847\\
587734949661769847&143.408040&9.85727&0.04917&$-19.61$&587734949661769846\\
587739406766375136&143.526352&27.34987&0.04252&$-20.17$&587739406766375135\\
587739114171728093&143.593216&29.22932&0.12847&$-21.39$&587739114171728095\\
587735343725805820&144.079695&9.32681&0.12569&$-21.92$&587735343725805821\\
587735343725805821&144.079950&9.32897&0.12507&$-21.60$&587735343725805820\\
587739116319998193&144.791689&31.35819&0.07704&$-20.19$&587739116319998186\\
588297863109017643&145.295662&39.00493&0.04571&$-19.85$&588297863109017642\\
587726033307238544&145.537540&2.47019&0.04935&$-20.08$&587726033307238543\\
587729388217303200&145.566609&54.31955&0.04674&$-19.60$&587729388217303201\\
587729388217303201&145.573340&54.31937&0.04674&$-19.09$&587729388217303200\\
587729385532489857&145.975999&52.07198&0.04564&$-19.63$&587729385532489855\\
588297864183283784&146.250980&40.18418&0.07280&$-20.35$&588297864183283785\\
588297864183283785&146.257288&40.18432&0.07302&$-20.08$&588297864183283784\\
587735661010747524&146.341730&34.70302&0.04091&$-19.17$&587735661010747523\\
587735661010747524&146.341730&34.70302&0.04091&$-19.17$&587735661010747525\\
587735661010747525&146.342201&34.69445&0.04053&$-18.80$&587735661010747523\\
587735661010747525&146.342201&34.69445&0.04053&$-18.80$&587735661010747524\\
587735661010747523&146.344435&34.70148&0.04014&$-18.87$&587735661010747524\\
587735661010747523&146.344435&34.70148&0.04014&$-18.87$&587735661010747525\\
587732483274703023&146.394648&42.87933&0.07336&$-20.13$&587732483274703029\\
587727944032649316&146.969222&2.20420&0.10013&$-20.98$&587727944032649315\\
588010137343688858&147.563272&57.76785&0.08265&$-20.77$&588010137343688856\\
587735662085341320&148.096529&36.29205&0.05891&$-19.77$&587735662085341319\\
587726033308352690&148.163735&2.59697&0.07296&$-20.26$&587726033308352692\\
587732579378462921&148.335482&6.88827&0.08934&$-20.69$&587732579378462922\\
588009366402302151&148.641693&56.55731&0.07390&$-20.31$&588009366402302152\\
587726033308680234&148.844975&2.57063&0.03167&$-18.85$&587726033308680320\\
587726033308680320&148.847270&2.58300&0.03142&$-19.35$&587726033308680234\\
588009365865365682&148.899493&56.04821&0.11582&$-21.25$&588009365865365683\\
588009365865365683&148.905641&56.04742&0.11743&$-21.32$&588009365865365682\\
587727942959693969&148.914494&1.59678&0.09867&$-21.35$&587727942959759366\\
587727942959759366&148.917693&1.59733&0.09862&$-20.90$&587727942959693969\\
587726032235200524&149.422641&1.76449&0.03128&$-18.78$&587726032235200533\\
587726032235200533&149.430391&1.75459&0.03169&$-19.16$&587726032235200524\\
587726033846009923&149.919215&3.02769&0.08014&$-20.72$&587726033846009924\\
587726033846075459&149.992617&3.04245&0.09060&$-20.57$&587726033846075458\\
587733081877708920&150.737096&50.84998&0.09240&$-20.95$&587733081877708919\\
587733080804032625&151.610537&50.11478&0.05038&$-19.33$&587733080804032623\\
587733080804032623&151.612443&50.10911&0.05041&$-19.82$&587733080804032625\\
587735660475908099&151.648420&36.24598&0.03108&$-18.93$&587735660475908100\\
587735660475908100&151.654604&36.25489&0.03036&$-18.34$&587735660475908099\\
587738946135195765&151.975294&34.03149&0.12564&$-21.65$&587738946135195766\\
587738946135195766&151.976297&34.03309&0.12726&$-21.73$&587738946135195765\\
587731869627056238&153.734583&51.13091&0.06771&$-19.94$&587731869627056237\\
587731869627056237&153.736576&51.12802&0.06774&$-20.34$&587731869627056238\\
587739407307505832&153.780536&31.12320&0.09092&$-20.75$&587739407307505833\\
587739407307505833&153.782076&31.12606&0.09124&$-20.57$&587739407307505832\\
588017977271386198&153.822229&34.53523&0.10100&$-20.82$&588017977271386199\\
587734863220244654&154.272464&8.85923&0.11498&$-21.25$&587734863220244656\\
587728879803629725&154.549206&4.07285&0.06169&$-19.98$&587728879803629729\\
588848900438491267&154.700071&0.38514&0.07094&$-21.02$&588848900438491268\\
588848900438491268&154.701081&0.38076&0.07066&$-20.27$&588848900438491267\\
588010360149049446&154.877252&5.01137&0.09984&$-20.93$&588010360149049445\\
588017978345652282&154.893013&35.67498&0.03780&$-19.03$&588017978345652278\\
588017978345652278&154.900801&35.68190&0.03837&$-19.40$&588017978345652282\\
587732135377961057&155.285192&48.48206&0.06180&$-19.68$&587732135377961058\\
587735349099954216&156.454156&13.75318&0.03186&$-19.39$&587735349099954217\\
588017703457390772&156.739749&11.00043&0.03211&$-18.23$&588017703457390781\\
588017703457390781&156.748774&10.99636&0.03198&$-18.67$&588017703457390772\\
587734948056858881&156.800096&10.32175&0.04878&$-19.76$&587734948056858885\\
587734948056858885&156.806469&10.32439&0.04908&$-19.86$&587734948056858881\\
587732048413065259&156.824154&53.19494&0.06393&$-20.04$&587732048413065260\\
587728950124478605&157.326074&0.97399&0.08933&$-20.65$&587728950124478604\\
587728950124478604&157.329867&0.97278&0.08862&$-21.12$&587728950124478605\\
588017977809830005&157.872291&35.91473&0.08903&$-21.07$&588017977809830004\\
588017977809830004&157.873277&35.91863&0.08796&$-20.83$&588017977809830005\\
588017977809830078&157.961955&35.96052&0.08756&$-20.53$&588017977809895502\\
588017977809895502&157.964208&35.96247&0.08676&$-20.51$&588017977809830078\\
588010359076880537&158.537755&4.35855&0.10044&$-21.32$&588010359076880538\\
588010359076880538&158.540361&4.35826&0.09964&$-21.70$&588010359076880537\\
587738948285432001&158.737242&37.73616&0.04292&$-18.87$&587738948285497349\\
587731869091758250&159.515178&52.14472&0.13776&$-21.70$&587731869091758251\\
588016891177074696&159.847442&39.08061&0.04315&$-20.30$&588016891177074695\\
587726033850400894&159.998216&3.11675&0.08531&$-21.11$&587726033850400895\\
587726033850400895&159.999293&3.11229&0.08396&$-21.62$&587726033850400894\\
587728309098708996&160.136747&2.48933&0.08152&$-20.51$&587728309098643602\\
587728879269314606&160.478039&3.83390&0.05602&$-20.79$&587728879269314607\\
587728879269314607&160.482444&3.83455&0.05580&$-20.19$&587728879269314606\\
587735661552992262&160.497092&39.44558&0.14836&$-21.74$&587735661552992264\\
588848900977983494&160.675736&0.68013&0.09454&$-20.66$&588848900977983495\\
588848901514920030&160.966484&1.06169&0.11595&$-21.74$&588848901514920032\\
588848901514920032&160.966895&1.06324&0.11779&$-21.18$&588848901514920030\\
587735661553188907&161.073063&39.70094&0.06818&$-20.63$&587735661553188906\\
587735661553188906&161.074078&39.70285&0.06944&$-21.23$&587735661553188907\\
587735661016318067&161.270053&39.33357&0.03499&$-19.56$&587735661016318066\\
587728950126706821&162.359594&1.01160&0.10704&$-21.42$&587728950126706822\\
588017606287949990&162.495562&43.97110&0.07949&$-21.02$&588017606287949989\\
588017606287949989&162.496398&43.97383&0.07875&$-20.35$&588017606287949990\\
587732577774534809&163.782733&6.69956&0.04582&$-19.21$&587732577774534817\\
587731498651680879&165.889777&54.77748&0.07564&$-20.42$&587731498651680880\\
587728309101265058&166.035894&2.59442&0.08106&$-20.50$&587728309101265059\\
588297864190099467&166.106892&45.78169&0.14292&$-21.94$&588297864190099466\\
587728308564459725&166.243505&2.31895&0.10097&$-21.18$&587728308564459726\\
587728308564459726&166.247003&2.31760&0.10045&$-20.80$&587728308564459725\\
588017719565156432&166.474236&39.78248&0.09907&$-20.96$&588017719565156433\\
587738618098352162&166.652033&37.00535&0.02656&$-18.08$&587738618098352161\\
588009370150568045&167.218552&60.13712&0.04516&$-20.29$&588009370150568046\\
587732772659789951&167.723402&10.53044&0.06885&$-20.76$&587732772659789950\\
587732772659789950&167.724872&10.53166&0.06844&$-20.76$&587732772659789951\\
587738616488198302&168.308653&36.01662&0.07872&$-20.41$&587738616488198303\\
588017110217785429&169.539017&45.61869&0.11112&$-21.45$&588017110217785430\\
588017110217785430&169.542280&45.62018&0.11076&$-21.17$&588017110217785429\\
588017721176948782&169.779420&41.50406&0.09418&$-20.68$&588017721176948783\\
587733081346211939&170.042475&54.60860&0.07083&$-20.60$&587733081346211938\\
587733081346211938&170.044099&54.60565&0.07022&$-20.75$&587733081346211939\\
587733080272404610&170.135706&53.80202&0.09990&$-20.83$&587733080272404611\\
588848899908370505&170.237764&-0.08438&0.02531&$-18.75$&588848899908370674\\
588848899908370674&170.239027&-0.09709&0.02534&$-18.26$&588848899908370505\\
587733080809472085&170.734968&54.23095&0.07215&$-20.03$&587733080809472086\\
587722984420409358&170.769674&0.86542&0.07149&$-20.40$&587722984420409360\\
587722984420409360&170.772686&0.86092&0.07186&$-21.04$&587722984420409358\\
587722984420409430&170.832775&1.02138&0.07435&$-21.03$&587722984420409431\\
587722984420409431&170.836165&1.02380&0.07459&$-20.65$&587722984420409430\\
587732583130529991&171.327423&59.94087&0.11346&$-21.07$&587732583130529989\\
587732583130529989&171.330686&59.94125&0.11265&$-21.43$&587732583130529991\\
588017719566794836&171.396682&40.50951&0.12269&$-21.27$&588017719566794837\\
588017720103731324&171.502970&40.90474&0.04491&$-19.29$&588017720103731326\\
588017720103731326&171.504937&40.90867&0.04606&$-19.38$&588017720103731324\\
587733081346605094&171.608536&54.79143&0.04636&$-19.17$&587733081346605098\\
587733080272994450&172.273189&54.09215&0.06915&$-20.70$&587733080272994451\\
587733080272994451&172.275398&54.09417&0.07051&$-20.87$&587733080272994450\\
587732580983111727&172.293670&58.37899&0.04143&$-18.81$&587732580983111734\\
587731870706106473&172.725797&55.62590&0.05348&$-19.79$&587731870706106474\\
587738946679800018&173.247105&38.91676&0.11026&$-21.38$&587738946679800019\\
587738946679800019&173.249046&38.91594&0.10911&$-20.97$&587738946679800018\\
588295841247658081&173.718442&49.23444&0.02964&$-18.34$&587732483283419240\\
587733081347195019&173.853418&54.96345&0.05550&$-19.62$&587733081347195018\\
587733081347195018&173.859674&54.95972&0.05423&$-19.91$&587733081347195019\\
587731870169497606&173.920373&55.18014&0.05807&$-20.93$&587731870169497605\\
587732483283550420&174.112495&49.47354&0.11797&$-21.19$&587732483283550419\\
588017605217943555&174.312813&44.77000&0.05797&$-19.61$&588017605217943556\\
587724650328359115&174.546712&-1.71567&0.07686&$-20.29$&587724650328359114\\
587731889503076531&174.738313&56.10334&0.09689&$-21.43$&587731889503076532\\
587731889503076532&174.739550&56.10170&0.09753&$-20.98$&587731889503076531\\
587733081347457227&174.996905&55.09803&0.05765&$-20.38$&587733081347457228\\
587733081347457228&175.005113&55.10272&0.05748&$-19.90$&587733081347457227\\
588010359621026002&175.254826&5.25558&0.03111&$-18.59$&588010359621026001\\
588010359621026001&175.256027&5.26026&0.03189&$-19.28$&588010359621026002\\
587725040089890968&175.436890&-2.74130&0.05461&$-20.63$&587725040089890969\\
587725040089890969&175.438876&-2.74158&0.05388&$-20.34$&587725040089890968\\
588011124648640608&175.626115&62.90270&0.09792&$-20.77$&588011124648640607\\
587739097523290296&176.113306&37.14453&0.11579&$-21.27$&587739097523290295\\
587739097523290295&176.113318&37.14220&0.11483&$-21.57$&587739097523290296\\
587738569236807847&176.533429&14.65507&0.06945&$-20.73$&587738569236807848\\
587738569236807848&176.537366&14.65324&0.06927&$-20.36$&587738569236807847\\
587733080274043068&176.538993&54.46586&0.07030&$-20.37$&587733080274043069\\
587739408389832835&176.661542&35.69536&0.07918&$-20.58$&587739408389832836\\
587735348034797608&176.703074&14.46928&0.07213&$-20.89$&587735348034797609\\
587735348034797609&176.706212&14.46618&0.07346&$-20.37$&587735348034797608\\
587732134847316170&177.112757&51.72260&0.13005&$-21.54$&587732134847316169\\
587738617565282329&177.555563&37.76966&0.05448&$-20.54$&587738617565282330\\
587735695368192087&177.559242&56.46528&0.06472&$-20.19$&587735695368257542\\
587735695368257542&177.565734&56.46353&0.06504&$-20.39$&587735695368192087\\
588017721179570246&177.604849&42.34808&0.08137&$-20.35$&588017721179570247\\
588295841785643112&177.689693&49.92287&0.03247&$-18.33$&588295841785643100\\
588017949886644381&177.800401&43.48930&0.07064&$-20.21$&588017949886644384\\
588017949886644384&177.804193&43.49450&0.07042&$-20.10$&588017949886644381\\
587731868559802396&177.873769&54.22489&0.06619&$-20.37$&587731868559802397\\
587731868559802397&177.877292&54.22358&0.06470&$-19.82$&587731868559802396\\
588010879831900245&177.888233&5.44831&0.12652&$-21.49$&588010879831900246\\
587739609698861151&178.662200&32.93099&0.07185&$-20.92$&587739609698861152\\
587739609698861152&178.664990&32.92978&0.07336&$-20.59$&587739609698861151\\
588009371226865738&178.695923&61.96704&0.15038&$-21.93$&588009371226865740\\
587735696979198021&178.725927&57.96723&0.10305&$-21.00$&587735696979198022\\
587731869633806414&178.798297&55.14071&0.05091&$-19.34$&587731869633806415\\
587731869633806415&178.801276&55.14775&0.05118&$-19.40$&587731869633806414\\
587733081885507678&179.532695&55.77466&0.05895&$-19.96$&587733081885507683\\
587733081885507683&179.542608&55.77216&0.05907&$-19.95$&587733081885507678\\
587722983887536152&179.978614&0.61696&0.10668&$-21.19$&587722983887536153\\
587732769980940318&180.503934&8.72386&0.05653&$-19.67$&587732769980940317\\
587732769980940317&180.506262&8.72808&0.05605&$-19.73$&587732769980940318\\
587733079201284216&180.517927&53.70877&0.06460&$-20.43$&587733079201284215\\
587733079201284215&180.522234&53.71348&0.06390&$-21.13$&587733079201284216\\
588009370690322557&180.524310&61.59824&0.09912&$-20.76$&588009370690322556\\
588009370690322556&180.527123&61.59941&0.09950&$-21.19$&588009370690322557\\
588017705078227047&180.532338&13.61061&0.08091&$-20.30$&588017705078227046\\
587731869097394331&180.745359&54.83716&0.04769&$-19.49$&587731869097394342\\
587731869097394342&180.755579&54.83150&0.04853&$-19.25$&587731869097394331\\
588013383816904793&181.158225&52.95477&0.08157&$-21.01$&588013383816904792\\
588013383816904792&181.164778&52.95730&0.08080&$-20.96$&588013383816904793\\
587739609699909692&181.523042&32.89306&0.02705&$-18.73$&587739609699909688\\
587731891115589739&182.367826&57.71623&0.04740&$-19.17$&587731891115589740\\
587739097525714956&182.984511&37.35274&0.08339&$-21.01$&587739097525714957\\
587738570850369571&183.406048&16.12169&0.02368&$-18.69$&587738570850369569\\
587738570850369569&183.415080&16.12525&0.02380&$-18.49$&587738570850369571\\
588017566026039378&183.591103&12.09056&0.06373&$-20.27$&588017566026039377\\
588017566026039377&183.594213&12.09165&0.06361&$-20.83$&588017566026039378\\
587738568166080683&183.689064&13.97505&0.08029&$-20.27$&587738568166080682\\
587738568166080682&183.690993&13.97513&0.08059&$-20.74$&587738568166080683\\
588017606295027743&185.225668&46.16169&0.03866&$-20.05$&588017606295027742\\
588017703469842606&185.734796&12.29230&0.09025&$-20.59$&588017703469842607\\
588017625082167414&186.674957&43.78232&0.11218&$-21.61$&588017625082167415\\
588017625082167415&186.676365&43.78447&0.11156&$-21.67$&588017625082167414\\
588017702933495938&187.028349&11.95531&0.08975&$-20.77$&588017702933495937\\
587739305291677774&187.419148&36.19941&0.07177&$-20.61$&587739305291677773\\
587739305291677773&187.423392&36.19808&0.07253&$-20.67$&587739305291677774\\
587732135924007022&188.043794&52.69565&0.05983&$-20.17$&587732135924007021\\
587726031715631234&189.073873&1.84675&0.07536&$-20.16$&587726031715631233\\
588017720109695168&189.633769&41.60033&0.06652&$-19.92$&588017720109695165\\
587726016684032064&190.201150&3.71840&0.07283&$-20.29$&587726016684032065\\
587735430151995577&190.243291&49.97563&0.11752&$-21.42$&587735430151995578\\
587724650872111259&190.263785&-1.28490&0.06371&$-20.13$&587724650872111260\\
587724650872111260&190.265147&-1.28605&0.06488&$-20.18$&587724650872111259\\
587738574335705187&190.397227&40.16669&0.08014&$-20.35$&587738574335705188\\
588017978358169768&190.944532&39.52974&0.10749&$-21.30$&588017978358169769\\
588017978358169769&190.945889&39.52898&0.10889&$-21.02$&588017978358169768\\
587722984429387944&191.358901&0.97673&0.08193&$-20.39$&587722984429387945\\
588848901528289406&191.438346&1.07987&0.10662&$-21.26$&588848901528289407\\
588017949891297351&192.439608&43.48239&0.06240&$-19.89$&588017949891297353\\
588010878764843115&193.118030&4.61277&0.08970&$-20.55$&588010878764843114\\
588010878764843114&193.118414&4.60997&0.08959&$-20.97$&588010878764843115\\
588011218595938370&193.134471&62.26327&0.10145&$-20.88$&588011218595938371\\
587725039560884369&193.314894&-3.17507&0.08449&$-20.78$&587725039560884370\\
587725039560884370&193.316647&-3.17681&0.08519&$-20.45$&587725039560884369\\
587724648189984811&195.317076&-3.47475&0.08629&$-21.04$&587724648189984812\\
587724648189984812&195.319520&-3.47323&0.08690&$-20.78$&587724648189984811\\
587736804545593530&195.982734&14.90170&0.03539&$-19.83$&587736804545593532\\
587736804545593532&195.983039&14.90721&0.03517&$-19.39$&587736804545593530\\
587738569245065342&196.057079&14.64044&0.14231&$-21.90$&587738569245065343\\
587732484363714609&197.031934&50.07970&0.05497&$-20.06$&587732484363714611\\
588017626159775840&199.043782&43.88332&0.09261&$-20.85$&588017626159775841\\
587732591182479485&199.272510&59.44265&0.11370&$-21.26$&587732591182479486\\
588848898847932529&200.502862&-0.85697&0.10642&$-21.13$&588848898847932530\\
587722982822772939&200.506097&-0.29930&0.07448&$-20.26$&587722982822772941\\
587722982822772941&200.507395&-0.30400&0.07453&$-20.31$&587722982822772939\\
587722982822903928&200.696040&-0.22991&0.08230&$-20.80$&587722982822903929\\
587722982822903929&200.698492&-0.23139&0.08182&$-20.45$&587722982822903928\\
588848900459200562&202.072151&0.28874&0.11086&$-21.77$&588848900459200563\\
588848900459200563&202.074003&0.28894&0.11007&$-21.48$&588848900459200562\\
587729777975951380&202.543025&-2.10501&0.08657&$-21.59$&587729777975951381\\
587729777975951381&202.545566&-2.10378&0.08631&$-21.50$&587729777975951380\\
587733411516645442&202.836180&54.09295&0.10567&$-20.98$&587733411516645443\\
587729772607045936&203.230301&-3.02635&0.04769&$-20.29$&587729772607045935\\
588018056720285950&204.131501&51.58379&0.06643&$-20.01$&588018056720351362\\
588018056720351362&204.141282&51.58437&0.06800&$-20.22$&588018056720285950\\
588011123044188183&205.208276&60.48091&0.04126&$-19.19$&588011123044188182\\
588011123044188182&205.211402&60.47869&0.04171&$-19.50$&588011123044188183\\
587732483829465169&205.762023&48.45824&0.08973&$-20.84$&587732483829465170\\
587735665841143833&206.292659&55.58226&0.06825&$-20.18$&587735665841143851\\
587735665841143851&206.300450&55.58417&0.06807&$-20.01$&587735665841143833\\
587735666915082252&207.394517&56.12610&0.13306&$-21.50$&587735666915082251\\
587735430694043762&207.996573&48.12472&0.06443&$-20.52$&587735430694043761\\
587735430694043761&207.999500&48.12062&0.06398&$-21.01$&587735430694043762\\
588017627236532460&208.546964&43.02415&0.11548&$-21.74$&588017627236532459\\
588017627236532459&208.548535&43.02344&0.11621&$-21.73$&588017627236532460\\
588848901536088292&209.262964&1.09168&0.10358&$-20.90$&588848901536088293\\
587736940369281226&209.453731&36.31288&0.06177&$-20.44$&587736940369281227\\
587736940369281227&209.454984&36.31877&0.06189&$-20.18$&587736940369281226\\
588017712048832731&209.631610&49.53710&0.10528&$-21.34$&588017712048832732\\
588017712048832732&209.631980&49.53981&0.10511&$-21.97$&588017712048832731\\
587735697523540143&210.236386&55.93418&0.10661&$-21.32$&587735697523540144\\
588011123582304321&210.743009&59.84182&0.07133&$-20.11$&588011123582304322\\
588017626163707946&210.807319&41.60952&0.03534&$-18.65$&588017626163707942\\
588017626163707946&210.807319&41.60952&0.03534&$-18.65$&588017626163707949\\
588017626163707949&210.816184&41.60377&0.03445&$-18.77$&588017626163707946\\
587726015619268767&210.865887&2.52881&0.07265&$-20.81$&587726015619268766\\
587726015619268766&210.866788&2.52488&0.07118&$-20.79$&587726015619268767\\
587729773147652315&211.779296&-2.58092&0.05694&$-20.68$&587729773147717749\\
587729773147717749&211.780016&-2.57785&0.05603&$-20.18$&587729773147652315\\
587736583889944596&211.958306&38.10695&0.06600&$-20.43$&587736583889944595\\
587726033873272951&212.261040&3.19156&0.08080&$-20.67$&587726033873272950\\
587726033873272950&212.261551&3.19425&0.08083&$-20.59$&587726033873272951\\
587735697524130068&212.382671&55.26478&0.04215&$-19.34$&587735697524130067\\
587735697524130067&212.388573&55.25904&0.04263&$-19.44$&587735697524130068\\
587729159511933072&214.494059&4.76641&0.08064&$-21.03$&587729159511933073\\
587729159511933073&214.497725&4.76642&0.08027&$-20.43$&587729159511933072\\
588298663046349038&215.317963&43.07083&0.10272&$-21.19$&588298663046349039\\
588017712587473124&215.527337&48.46405&0.07332&$-20.77$&588017712587473125\\
588017712587473125&215.532418&48.46846&0.07359&$-20.32$&588017712587473124\\
587729970712674574&216.139411&-2.52841&0.10864&$-20.99$&587729970712674575\\
587729971786481830&216.158081&-1.63228&0.05498&$-20.76$&587729971786481829\\
588848900466082030&217.744920&0.40669&0.13061&$-21.42$&588848900466082029\\
588848900466082029&217.745005&0.40462&0.13052&$-21.50$&588848900466082030\\
587729971787333683&218.154609&-1.52340&0.05254&$-19.43$&587729971787333864\\
587729971787333864&218.156514&-1.53012&0.05226&$-19.42$&587729971787333683\\
587726100948713690&218.518708&3.77571&0.02799&$-18.03$&587726100948713695\\
588011124121010348&218.547717&58.25537&0.13739&$-21.67$&588011124121010349\\
587736940372754584&218.725901&33.82626&0.05777&$-20.42$&587736940372754585\\
587736940372754585&218.727836&33.82223&0.05874&$-20.61$&587736940372754584\\
588017603622142042&219.496721&38.36513&0.03527&$-19.52$&588017603622142041\\
588017979979137119&220.286230&35.33301&0.07916&$-20.30$&588017979979137117\\
587733605331042485&221.003937&55.39655&0.07900&$-20.81$&587733605331042484\\
587733605331042484&221.012422&55.39660&0.08013&$-20.28$&587733605331042485\\
587729158978339151&222.078972&3.81497&0.02766&$-18.36$&587729158978339152\\
587729158978339152&222.080344&3.80839&0.02798&$-18.64$&587729158978339151\\
587733603184607460&222.933920&52.58642&0.06619&$-19.84$&587733603184607338\\
587733603184607338&222.944240&52.58628&0.06525&$-20.25$&587733603184607460\\
587726033341776175&224.590165&2.54692&0.02777&$-19.12$&587726033341776191\\
587726033341776191&224.596839&2.53856&0.02789&$-19.20$&587726033341776175\\
587735491359867067&227.156983&42.63435&0.15383&$-21.80$&587735491359867068\\
587729778523766950&227.547406&-1.19531&0.07085&$-21.26$&587729778523766951\\
587729778523766951&227.550388&-1.19089&0.07015&$-20.94$&587729778523766950\\
587726016163545219&227.795789&2.65396&0.04082&$-18.76$&587726016163545218\\
587735490286714916&228.023777&41.20996&0.02769&$-18.50$&587735490286714925\\
588017603625943177&229.307454&34.62073&0.06129&$-20.43$&588017603625943176\\
588017603625943176&229.309566&34.61728&0.06176&$-19.70$&588017603625943177\\
587733603723444349&229.336727&50.55268&0.07529&$-20.74$&587733603723444348\\
587733603723444348&229.340941&50.55065&0.07402&$-20.52$&587733603723444349\\
588017604163010684&229.768827&34.65395&0.07575&$-20.93$&588017604163010685\\
588017604163010685&229.773990&34.65459&0.07489&$-20.24$&588017604163010684\\
587736586044178565&230.182440&33.41340&0.08060&$-20.67$&587736586044178566\\
587733399176740884&230.236555&45.72180&0.02713&$-19.00$&587733399176740883\\
587722983372751055&230.351281&0.11415&0.07616&$-20.86$&587722983372751056\\
587722983372751056&230.351544&0.11712&0.07611&$-20.42$&587722983372751055\\
588017978909851719&231.011770&30.24459&0.06216&$-20.16$&588017978909851720\\
587736618783998122&231.208934&31.69386&0.08198&$-21.08$&587736618783998123\\
587736618783998123&231.212919&31.69710&0.08025&$-20.80$&587736618783998122\\
587725818033799200&231.698953&59.26291&0.04465&$-20.36$&587725818033799199\\
588011102640930946&232.081687&53.06304&0.05322&$-20.04$&588011102640930960\\
588011102640930960&232.093595&53.06088&0.05273&$-20.13$&588011102640930946\\
587729158982860843&232.377532&3.28562&0.09822&$-20.83$&587729158982860844\\
588018090004775179&234.959647&34.65827&0.02160&$-18.22$&588018090004774979\\
588017603628564733&235.326271&31.46862&0.05446&$-19.54$&588017603628564734\\
588017603628564734&235.327513&31.47294&0.05590&$-20.17$&588017603628564733\\
588018090006085868&237.834899&32.89637&0.11208&$-21.38$&588018090006085870\\
587736619323687149&237.946205&28.86063&0.07719&$-20.54$&587736619323687150\\
587736619324014665&238.587194&28.30914&0.07896&$-21.43$&587736619324014666\\
587736619324014666&238.588375&28.31049&0.07772&$-20.86$&587736619324014665\\
587736619324014711&238.638473&28.32982&0.07803&$-20.47$&587736619324014712\\
587736941991559337&238.928782&26.70544&0.08312&$-20.79$&587736941991559340\\
588017979987067206&239.326975&27.07408&0.06828&$-20.10$&588017979987067207\\
588017979987067207&239.330862&27.07124&0.06777&$-20.55$&588017979987067206\\
587736783068921889&239.603774&35.14779&0.04624&$-19.66$&587736783068921888\\
587736783068921888&239.606303&35.15205&0.04575&$-19.93$&587736783068921889\\
587736584438087878&239.666668&26.97766&0.06429&$-21.00$&587736584438087879\\
587736898502394212&245.013669&26.05191&0.13279&$-21.49$&587736898502394213\\
587736919434789305&245.487737&25.69153&0.09948&$-20.96$&587736919434789306\\
587736619327619466&246.275178&23.66915&0.06471&$-20.34$&587736619327619485\\
587736619327619485&246.281423&23.66696&0.06472&$-19.92$&587736619327619466\\
587729652884898167&247.721313&41.28636&0.09361&$-20.67$&587729652884898166\\
587729651811746014&247.823595&39.79398&0.02916&$-18.90$&587729651811746015\\
587729651811746015&247.831559&39.79050&0.02897&$-19.09$&587729651811746014\\
588018056200716579&249.067768&29.98005&0.09677&$-20.76$&588018253762593037\\
587736920510169204&249.160662&23.83123&0.04537&$-19.51$&587736920510169203\\
587736920510169203&249.162457&23.82895&0.04570&$-19.37$&587736920510169204\\
587735744231112813&249.738926&25.94776&0.12921&$-21.77$&587736751935914045\\
587736751935914045&249.739344&25.95011&0.12862&$-21.70$&587735744231112813\\
587736919974084982&250.404688&22.44180&0.12048&$-21.27$&587736919974084981\\
587736585517007021&250.736068&20.66155&0.08178&$-20.38$&587736585517007020\\
587733603733864744&251.801970&33.30575&0.05372&$-19.94$&587733603733864746\\
587733603733864746&251.807035&33.30564&0.05295&$-19.47$&587733603733864744\\
587736782001799572&252.023515&24.33744&0.03631&$-19.03$&587736782001799335\\
587736782538735817&252.448588&24.50495&0.05708&$-19.70$&587736782538735818\\
587733398114009448&252.770035&27.79932&0.11018&$-21.11$&587733398114009447\\
587733398114009447&252.774282&27.79865&0.11128&$-21.15$&587733398114009448\\
587729652352614489&254.730794&32.51305&0.06029&$-20.61$&587729652352614488\\
587729652352614488&254.735606&32.51551&0.06062&$-20.09$&587729652352614489\\
588018055130710322&255.028671&23.13151&0.05683&$-20.39$&588018055130710321\\
588018055130710321&255.029227&23.12753&0.05679&$-19.76$&588018055130710322\\
587729752747147785&255.514361&33.64516&0.09638&$-20.82$&587729752747147786\\
587729752747278350&255.637425&33.50498&0.08440&$-20.48$&587729752747278349\\
587729653963030855&255.742715&33.58123&0.08675&$-20.67$&587729653963030857\\
587733432998297780&255.765897&25.52968&0.03169&$-18.77$&587733432998297779\\
587733432998297779&255.771201&25.52990&0.03145&$-18.48$&587733432998297780\\
587733398652518655&255.896222&25.34918&0.03793&$-18.88$&587733398652518656\\
587733398652518656&255.898962&25.34741&0.03846&$-18.80$&587733398652518655\\
587729781199667608&256.008867&33.87058&0.09116&$-21.15$&587729781199667607\\
587729781199667607&256.010966&33.86885&0.09145&$-21.51$&587729781199667608\\
587725503946293263&256.157111&60.58514&0.09684&$-20.84$&587725503946293264\\
587729407545967181&256.207559&33.41226&0.08358&$-20.54$&587729781199864370\\
587729781199864370&256.209455&33.41212&0.08270&$-20.38$&587729407545967181\\
587729408619184367&256.212001&34.81472&0.05725&$-20.49$&587729408619184366\\
587729408619184366&256.212288&34.81734&0.05635&$-20.79$&587729408619184367\\
587729408083034337&256.749917&33.17156&0.08219&$-20.36$&587729408083034334\\
587729409157825092&259.101916&31.57673&0.07909&$-20.28$&587729409157825093\\
587725590381920321&259.315611&64.26116&0.03465&$-18.84$&587725590381920320\\
587725590381920320&259.322265&64.27001&0.03408&$-19.25$&587725590381920321\\
587725491063488610&259.646698&56.05713&0.02966&$-19.19$&587725491063488609\\
587725491063488609&259.647074&56.06115&0.03021&$-18.79$&587725491063488610\\
587725589311979806&262.588367&55.77737&0.11297&$-21.12$&587725589311979807\\
587730848499237584&315.922756&0.92776&0.04872&$-19.51$&587730848499237585\\
587731173844451913&317.323508&0.27197&0.05001&$-20.09$&587731173844451548\\
587731173844451548&317.323984&0.26460&0.05077&$-19.73$&587731173844451913\\
587731187798507929&323.407522&1.07095&0.08602&$-21.38$&587731187798507928\\
587731187798507928&323.410208&1.06867&0.08596&$-21.48$&587731187798507929\\
587730847966167546&324.572783&0.51841&0.04130&$-18.79$&587730847966167545\\
587730847966167545&324.573469&0.52104&0.04181&$-18.87$&587730847966167546\\
587731185114677697&324.653293&-0.94348&0.08388&$-20.40$&587731185114677696\\
587730817895563468&329.713600&-7.66075&0.09909&$-21.23$&587730817895563467\\
587731187268190294&338.411394&0.67136&0.06115&$-20.04$&587731187268190295\\
587731187268190295&338.415866&0.66980&0.06170&$-20.11$&587731187268190294\\
587730774953492889&338.808693&14.07062&0.08341&$-21.00$&587730774953492888\\
587730774953492888&338.812759&14.06910&0.08234&$-20.97$&587730774953492889\\
587731186195235018&340.122898&-0.06242&0.05940&$-19.65$&587731186195235014\\
587727874768371831&351.221554&-9.90745&0.06992&$-20.10$&587727874768371832\\
587727874768371832&351.223714&-9.90925&0.06977&$-20.33$&587727874768371831\\
587727873696399447&355.370638&-10.72577&0.08910&$-20.90$&587727873696399448\\
587727873696399448&355.370841&-10.72436&0.08934&$-20.61$&587727873696399447\\
%\input{hosts}
\tableline
\end{tabular}
\end{center}
\end{table}


